Constraining Light Thermal Inelastic Dark Matter with NA64

A vector portal between the Standard Model and the dark sector is a predictive and compelling framework for thermal dark matter. Through co-annihilations, models of inelastic dark matter (iDM) and inelastic Dirac dark matter (i2DM) can reproduce the observed relic density in the MeV to GeV mass range without violating cosmological limits. In these scenarios, the vector mediator behaves like a semi-visible particle, evading traditional bounds on visible or invisible resonances, and uncovering new parameter space to explain the muon $(g-2)$ anomaly. By means of a more inclusive signal definition at the NA64 experiment, we place new constraints on iDM and i2DM using a missing energy technique. With a recast-based analysis, we contextualize the NA64 exclusion limits in parameter space and estimate the reach of the newly collected and expected future NA64 data. Our results motivate the development of an optimized search program for semi-visible particles, in which fixed-target experiments like NA64 provide a powerful probe in the sub-GeV mass range.

==> authorlist.tex <==
\author{
Martina~Mongillo\thanksref{addrETH,e1}\and
Asli~Abdullahi\thanksref{addrFNAL,addrDH}\and
Benjamin~Banto~Oberhauser\thanksref{addrETH}\and
Paolo~Crivelli\thanksref{addrETH,e4}\and
Matheus~Hostert\thanksref{addrW, addrSPA_MN,addrWIFTPI_MN}\and
Daniele~Massaro\thanksref{addrBO,addrINFN, addrLU}\and
Laura~Molina~Bueno\thanksref{addrVA}\and
Silvia~Pascoli\thanksref{addrBO,addrINFN}
}

\thankstext{e1}{e-mail: mmongillo@student.ethz.ch (corresponding author)}
\thankstext{e4}{e-mail: Paolo.Crivelli@cern.ch (corresponding author)}
%\thankstext{e2}{e-mail: asli.abdullahi@durham.ac.uk}
%\thankstext{e3}{e-mail: bantoobb@student.ethz.ch}
%\thankstext{e5}{e-mail: mhostert@pitp.ca}
%\thankstext{e6}{e-mail: daniele.massaro5@unibo.it}
%\thankstext{e7}{e-mail: laura.molina.bueno@cern.ch}
%\thankstext{e8}{e-mail: silvia.pascoli@unibo.it}

\institute{
Institute for Particle Physics and Astrophysics, ETH Z\"urich,
Z\"urich, CH-8093, Switzerland \label{addrETH}
\and
Theoretical Physics Department, Fermi National Accelerator Laboratory, Batavia, IL 60510, USA  \label{addrFNAL}
\and
Institute for Particle Physics Phenomenology, Department of Physics, Durham University, South Road, Durham DH1 3LE, United Kingdom  \label{addrDH}
\and
Perimeter Institute for Theoretical Physics, Waterloo, ON N2J 2W9, Canada  \label{addrW}
\and
School of Physics and Astronomy, University of Minnesota, Minneapolis, MN 55455, USA \label{addrSPA_MN}
\and
William I. Fine Theoretical Physics Institute, School of Physics and Astronomy, University of Minnesota, Minneapolis, MN 55455, USA \label{addrWIFTPI_MN}
\and
Dipartimento di Fisica e Astronomia, Universit\`a di Bologna, via Irnerio 46, 40126 Bologna, Italy \label{addrBO}
\and
INFN, Sezione di Bologna, viale Berti Pichat 6/2, 40127 Bologna, Italy \label{addrINFN}
\and
Centre for Cosmology, Particle Physics and Phenomenology (CP3), Universit\'e Catholique de Louvain, B-1348 Louvain-la-Neuve, Belgium \label{addrLU}
\and
Instituto de Fisica Corpuscular (CSIC/UV),
Carrer del Catedrátic José Beltrán Martinez, 2, 46980 Paterna, Valencia, Spain \label{addrVA}
%\and
%CERN, Theoretical Physics Department, Geneva, Switzerland %\label{addrCERN}
}
